Parametric Graph Templates: Properties and Algorithms

Hierarchical structure and repetition are prevalent in graphs originating from nature or engineering. These patterns can be represented by a class of parametric-structure graphs, which are defined by templates that generate structure by way of repeated instantiation. We propose a class of parametric graph templates that can succinctly represent a wide variety of graphs. Using parametric graph templates, we develop structurally-parametric algorithm variants of maximum flow, minimum cut, and tree subgraph isomorphism. Our algorithms are polynomial time for maximum flow and minimum cut and are fixed-parameter tractable for tree subgraph isomorphism when parameterized by the size of the tree subgraph. By reasoning about the structure of the repeating subgraphs, we avoid explicit construction of the instantiation. Furthermore, we show how parametric graph templates can be recovered from an instantiated graph in quasi-polynomial time when certain parameters of the graph are bounded. Parametric graph templates and the presented algorithmic techniques thus create opportunities for reasoning about the generating structure of a graph, rather than an instance of it.

==> sec-sibling.tex <==
\section{Extensions: Sibling Edges}

%\paragraph{Acyclic parametric.}
%An \emph{acyclic parametric graph} is a parametric graph where none of its instantiations contains a cycle \emph{and} it is intra-template acyclic.

%For a template $M_i$, the set of nodes in $M_i$ that have incoming edges from outside the template are the \emph{entry nodes} of the template $M_i$ (i.e. the set of nodes $v \in M_i$ with $(u, v)\in E$ and $u\not \in M_i$). 

%Similarly, for a template $M_i$, the set of nodes in $M_i$ that have outgoing edge to outside the template are the \emph{exit nodes} of the template $M_i$ (i.e. the set of nodes $u \in M_i$ with $(u, v)\in E$ and $v\not \in M_i$).

%(We will generally require that the set of entry nodes and exit nodes for a template are disjoint.)

\paragraph{Sibling Edges}

So far, there are no edges between instances of the same template. We can extend the model by allowing an instance to have edges \emph{to another instance of the same template}. These edges can for example model sequential chains (pipelines), convolutional networks, and grids. We call these edges \emph{sibling edges} (because they connect siblings). %A pparametric graph with pipes is called \emph{piped}.

A \emph{sibling edge} (u,v) of template $T_i$ connects (in the template graph of $T_i$) a vertex $u$ that belongs to template $T_i$ to a vertex $v$ that \emph{also} belongs to $T_i$. Every sibling edge  $e=(u,v)$ of template $T_i$ is associated with a \emph{bijective} (and computable) \emph{sibling function} $f_e : \{0, \dotsc, P_i-1\} \rightarrow \{0, \dotsc, P_i-1\}$ which tells us that if the head of edge $e$ is in instance $j$ of the template $T_i$, then the tail of edge $e$ is in instance $f(j)$ of the template $T_i$.
\yishai{Not sure if the \(O(1)\)-computable aspect is important here. In graph terms this is just a fixed label on each node...} \lukas{It is important if we evaluate $f$ during our algorithms. Also, if the function is not efficiently computable, there is no way to instantiate the graph efficiently, which undoes the whole point of representing it as a parametric graph}
%
Unless otherwise stated, we assume sibling functions for an edge $e$ in template $T_i$ are of the form $$f_e(x)=x+\Delta \mod P_i$$ for some integer $\Delta$. This ensures that the problems are symmetric from every instances point of view.

Examples.
Overview of Techniques.

\subsection{BFS}

Breath-First Search (BFS) is one of the most fundamental graph algorithms. It's generalization to parametric graphs will form the basis for several of our more involved algorithms, like those for maximum flows (\Cref{sec:stflow}) and tree subgraph isomorphism (\Cref{sec:tree-si}). It also provides a solution to single-source shortest paths (\Cref{sec:sssp})
%
A parametric graph that is acyclic \emph{and} template-acyclic is \emph{strongly template-acyclic}.
%
This section focuses on the case of \emph{strongly acyclic} parametric graphs.

The algorithm uses the idea of \emph{partial instantiation}. This algorithmic design principle is about explicitly instantiating a crucial subset of the instances, and dealing with the remaining instances in an efficient manner. Which instances are crucial and how to deal with the remaining instances depends on the specific graph problem. The main point of partial instantiation is to deal with the sibling edges.

\subsection{The Jump Graph}\label{sec:jump-graph}

The idea is to characterize the set of \emph{reachable instances} from a given vertex via paths in a so-called \emph{jump graph}. We will first describe the naive construction for the jump graph and then show how to reduce the size of the jump graph.

The \emph{jump graph} of a template $T$ is a weighted, directed graph derived from the template graph of $T$ (it has the same set of vertices and edges). The weight of a sibling edge $e$ where both endpoints belong to $T$ is $w(e)=f_e(i)-i$. This is the amount a sibling edge "jumps" between instances. The weight of other edges in the jump graph is $0$.

The jump graph characterizes which instances of which vertices are reachable:
\begin{observation}\label{obs:jump-graph}
	Consider a template $T_i$ where there is no cycle in the template graph of its parametric graph that contains both vertices that belong to $T_i$ and vertices that do not. Then, there is a path from instance $i$ of vertex $x$ to instance $j$ of vertex $y$ in the instantiated graph if and only if there is a walk from $x$ to $y$ in the jump graph of $T_i$ of weight $j-i \pmod {P_i}$.
\end{observation}
Note that the condition of the observation is trivially satisfied in strongly acyclic graphs (we will also use jump graphs for connectivity in the undirected case in \Cref{sec:connected-components}, where the observation will hold on certain subgraphs of the template graph).

The jump graph has the same size as the template graph, which is too big for our purposes (as we will get runtimes that are in the worst case exponential in the size of the jump graph). Thus, we show how to \emph{shrink} the jump graph.

\paragraph{Shrinking the jump graph} Vertices that are not adjacent to any sibling edge do not contribute much useful information to the jump graph. They can be removed as long as the set of vertices reachable through zero-weight edges remains preserved. In the applications of the jump graph there is a special query vertex $v$ from which the reachable instances are determined.

The \emph{shrinked jump graph} contains the vertices of the jump graph which are incident to at least one nonzero-weight edge. It also contains the query vertex $v$. Every nonzero-weight edge in the jump graph is also in the shrinked jump graph. There is a weight-zero edge between a vertex $u$ and a vertex $v$ in the shrinked jump graph if and only if there is a path from $u$ to $v$ \emph{using only weight zero edges} in the jump graph.

The set of weight zero edges in the shrinked jump graph can be determined by doing a breadth first search in the subgraph of the jump graph consisting of only weight $0$ edges from every vertex that is in the shrinked jump graph.

Let $x$ be the number of sibling edges in the template $T_i$. Then, its shrinked jump graph has at most $2x+1$ vertices and $O(x^2)$ edges. Constructing it takes $O(m_i x)$ time.

\paragraph{The set of reachable instances.} The set of reachable instances from a vertex $v$ is given by the lengths of all paths in the shrinked jump graph, by \Cref{obs:jump-graph}.

If the shrinked jump graph is acyclic, the set of all path lengths from a vertex $v$ can be determined by traversing the shrinked jump graph in topological order from $v$. For every vertex $v$, a set $I(v)$ of path lengths is computed. When visiting a vertex $u$ where the neighbors of $u$ prior in the topological order are $p_1, \dotsc, p_k$, every path already found for such a neighbor is extended by the edge connecting it to $u$, respectively. That is, we set $$I(u) = \cup_i \{ j+ w(p_i, u) \ | \ j \in I(p_i)\} \enspace .$$

The size of the sets $I(u)$ is bound by the total number $k$ of $v-u$ paths over all $u$ in the shrinked jump graph. In the worst case, there can be at most $2^{k}$ paths in an acyclic graph of $k$ vertices, because every subset of vertices defines at most one path. Thus, the algorithm takes $O(x2^{2x})$ time in the worst case.

Alternatively, we can provide a \emph{pseudo-polynomial} time bound in the total absolute weight of the jump graph $\delta$. Observe that the sets $I(u)$ have size at most $\delta$ for every vertex because they correspond to weights of paths in the jump graph. Hence, the algorithm takes time at most $O(x^2 \delta )$.

\begin{lemma}[Reachable Instances]
Determining the set of reachable instances of a template $T_i$ (satisfying the conditions of \Cref{obs:jump-graph}) takes $O(x\min( x \delta, 2^{2x}) + m_i x)$ time, where $x$ is the number of sibling edges and $\delta$ is their total absolute weight $\sum_e |f_e(i)-i)|$.
\end{lemma}


\subsection{Upwards Partial Instantiation} \label{sec:partial-instantiation-siblings}

The set of instances reachable from a vertex $v$ considering only instances of templates that are $T(v)$ or ancestors thereof can be found by computing reachable instances starting with $T(v)$ and walking up the template hierarchy. %efficiently - if the largest number of sibling edges in any template $x$ is small, i.e. $O(\log n)$. In particular, it takes $O(m 2^{2x})$ time.

Proceed iteratively until having processed the root template.
\begin{enumerate}
	\item Start with determining the set of instances reachable in the template $T(v)$ that $v$ belongs to (using the Shrinked Jump graph).
	\item Instantiate these reachable instances (choosing parameter $1$ for all descendant templates) and determine which exit nodes $V'$ of $T(v)$ are reachable. 
	\item Delete the template $T(v)$ and replace it by a single dummy vertex $v$ connected to all exit nodes $V'$.
\end{enumerate}
Then, partially instantiate the graph according to the visited set of instances.

\begin{lemma}
Instantiating all instances reachable from a vertex $v$ using only edges that do not descend in the template hierarchy in a parametric graph takes $O(m x \min(x\delta,  2^{2x}))$ time.%, where $x$ is the largest number of sibling edges in any template.
\end{lemma}

\subsection{Parametric Graph Template of the BFS Tree}

After partial instantiation starting form the root vertex $s$, only templates that are descendants of an ancestor of $T(s)$ remain. Since each of the instances of such templates behave completely symmetrically with respect to the root $s$, they can be treated as though they are instantiated only once. The BFS tree computed on the resulting graph will provide a \emph{parametric graph template for the BFS tree} of the instantiated graph.  %We show that these templates can be merged with their  %t turns out that these templates can be treates as though all their vertices belong to the template that is the least common ancestor of t 

\paragraph{BFS: Partial Instantation Algorithm}
\begin{enumerate}
	\item Do a partial upwards instantiation starting from the root $s$.
	\item Perform a BFS from the root in the partially instantiated graph.
	\item Add the templates that are descendants of a partially instantiated template to this BFS tree. This gives a parametric graph for the BFS tree.
\end{enumerate}


\begin{theorem}
	Constructing a parametric graph template of the BFS tree of a strongly acyclic parametric graph takes $O(m x\min( x \delta, 2^{2x}))$ time.%, where $x$ is the largest number of sibling edges in any template.
\end{theorem}

\paragraph{Correctness} We argue that descendants of a partially instantied templates are handled correctly.

%If the root of the tree is in the root template, then the BFS tree of the template graph is a template for the BFS tree of the instantiated graph. This can be generalized so that whenever the root is in an ancestor of a template, looking at the template graph of this template suffices. This will deal with the remaining templates.
\begin{observation}\label{obs:paths-correspondence}
	There is a path between vertex $u$ and $v$ in the template graph if and only if there is a path between an instance of $u$ and an instance of $v$.
\end{observation}
\begin{proof}
	There is an edge from vertex $x$ and to vertex $y$ in the template graph if and only if there is an edge from an instance to $x$ to an instance of $y$. Hence, we a path from $u$ to $v$ in the instance corresponds to a walk from $u$ to $v$ in the template. Therefore, there's also a path from $u$ to $v$. The other direction is easy because a path in the template always corresponds to a path in the instantiated graph.
\end{proof}

\begin{observation}\label{obs:arborescence}
Consider a template graph $G$ that is a directed tree rooted at a vertex $v$ that reaches vertices $V'$. If $v$ belongs to the root template, the instantiation of $G$ is a directed tree rooted at $v$ that reaches every instance of every vertex in $V'$.
\end{observation}
\begin{proof}
The instantiation of a directed tree is acyclic. Otherwise, consider a cycle $v_1, v_2, \dotsc, v_k, v_1$ in the instantiated tree. This cycles gives a cycle in the template graph: Map the cycle $v_1, v_2, \dotsc, v_k, v_1$ to a walk in the template graph by mapping every instance of a vertex to the vertex that instantiated it. This is a closed walk. Hence, there is a cycle in the template graph, which is a contradiction. % cycle goes from an instance of $x$ to an instance of $y$, move from $x$ to $y$.

Moreover, the instantiation of the directed tree has maximum in-degree $1$. This follows from the bijectivity of the sibling function.

Finally, there is a path from the root $v$ to every other instances of every vertex in $V'$ because of \Cref{obs:paths-correspondence}.
\end{proof}
To obtain the desired result, treat every partially instanted template as its own root template.



\subsection{Single-Source Shortest Paths} \label{sec:sssp}

Essentially the same idea also works to construct a template for the single-source shortest path tree (which allows us to determine the distance from a source to every target in the instantiated graph):

Upwards-partially instantiate all instances reachable from the source vertex. Then, run a single-source shortest path algorithm on the partially instantiated graph constructing a shortest-path tree. Add back again the templates that are descendants of the partially instantiated templates.

\begin{theorem}
	Constructing a parametric graph template of the SSSP tree of a strongly acyclic parametric graph takes $O(m2^{2x})$ time, where $x$ is the largest number of sibling edges in any template.
\end{theorem}

The correctness follows by dividing every weight $w$ edge into $w$ successive unweighted edges and observing that the BFS algorithm produces the analogous result.% Do not need to do this explicitly, just use a DP algorithm for the distances/distance tree. Same runtime as the BFS.

Note that because the instantiated graph is acyclic, its shortest path tree can be found in linear time in its size.



\subsection{Connected Components} \label{sec:connected-components}

\lukas{transition}

We consider an undirected parametric graph and want to know the number of connected components in an instantiated graph. Note that a connected template graph can give rise to a disconnected instantiated graph in the presence of sibling edges.

\begin{theorem}
	The number of connected components of the instantiation of a parametric graph can be determined in $O(m \log \delta)$ time, where $\delta$ is largest total absolute weight of the jump graph.
\end{theorem}

The following shows that we can easily reduce the problem to computing the number of connected components of a single template with a connected template graph:


\begin{enumerate}
	\item Traverse the template tree bottom-up. When visiting template $T$, merge all vertices that belong to $T$ and have a path to a boundary vertex.
	\item Then, put every connected component of a template graph into its own template.% \yishai{How can a vertex in \(T\) not have a path to a boundary vertex? Is this even possible/meaningful?} \lukas{we want to be as general as possible here, because CC appears as a subroutine of other algorithms, so we might be looking at a disconnected sub graph template}
For each such resulting template $T`$, compute its number of connected components and multiply this result by the product of the parameters of the templates that contain the template $T`$.
\end{enumerate}

We next focus on the case of a single template with connected template graph. As in acyclic directed connectivity (\Cref{sec:jump-graph}), we will use the jump graph to characterize the set of reachable instances for a single template. However, we can exploit that we are in the undirected case by \emph{contracting} all non-sibling edges in the jump graph. This would leave a graph with $O(x)$ vertices and $O(x)$ edges. Recall that the reachability algorithm from \Cref{sec:jump-graph} relied on the jump graph being acyclic, which is not the case for our setting here. Thus, we need to consider walks (actually \emph{closed walks}) to determine the connected components.

It is enough to consider \emph{linear combinations of cycles (and loops)} to characterize all the closed walks. Also note that if there is a closed walk of weight $k$ in the jump graph, then for every vertex $v$ there is also a closed walk of weight $k$ that contains the vertex $v$.

\begin{lemma}
	In the jump graph of template $T_i$ there is a closed walk of  weight $k$ (modulo $P_i$) if and only if there is a linear combination of cycles and loops in the jump graph of combined weight $k \pmod {P_i}$.
\end{lemma}

We can use the following characterization of linear congruence equations to decide if a certain linear combination of cycles is possible (modulo $P_i$):
\begin{lemma}
	The linear congruence equation $\sum_{i=1}^{k} a_i x_i \equiv_p b$ with variables $x_1, \dotsc, x_k$ has solutions if and only if \(\gcd{\left(a_1, \dotsc, a_k, p\right)}\) divides $b$.
\end{lemma}
Euclid's algorithm determines the greatest common denominator of two numbers $a$ and $b$ using $O(\log a)$ arithmetic operations ($a<b$)~\cite{TODO}.
The problem remains that we might need to look at all cycles in a graph of $O(x)$ vertices, which could be $2^x$ in the worst case.

\subsection{Retemplating}

It is possible to transform any template with connected template graph into a template where the template subgraph consisting only of non-sibling edges is connected. It is much easier to answer the question regarding the number of connected components of the instance of this template, because all vertices can be merged into a \emph{single vertex}. Thus, all closed walks consist of a sequence of loops, which we can enumerate in linear time.

\begin{lemma}(Retemplating)
Given a connected template graph with a single template, we can construct in $O(m)$ time a template graph that instantiates isomorphic graphs (for all parameters) where the template graph without sibling edges is connected.
\end{lemma}

\paragraph{Retemplating Algorithm.} \lukas{picture}
The idea is that we can take any spanning tree (of the jump graph) as the set of non-sibling edges and adjust the sibling functions of all other edges accordingly.

For simplicity, we consider all arithmetic modulo the parameter $P$, so that $P+k = k$ for all $k>1$ and we avoid writing the modulo explicitly.

\begin{enumerate}
	\item Compute a spanning tree $A$ of the jump graph. For the spanning tree computation, ignore the edge directions, but represent $A$ as a weighted directed graph where the weight of an edge $(u,v)$ is the same as it is in the jump graph, i.e. $w(u,v)=-w(v,u)$.
	\item  Create a new template $T'$ from $T$ with the same vertices, but different sibling edges and sibling edge functions. All edges in the spanning tree $A$ are non-sibling edges in $T'$.
	\item All other edges are sibling edges in $T'$. Say the edge $e=(u, v)$ has length $\Delta$ in the jump graph of $T$. Compute the weight $\gamma(v, u)$ of the path from the vertex $v$ to the vertex $u$ in the tree $A$. The edge $e=(u,v)$ has sibling function $f_e(i)=i+\Delta+\gamma$.
\end{enumerate}
This transformation can be implemented in $O(m)$ time: root the tree $A$ and then compute for each vertex the sum of the weights along the path from the vertex to the root by traversing the tree in DFS order and keeping a running sum. Let $\alpha(i)$ be the sum of the weights from vertex $i$ to the root along $A$. Then, we can see that $\gamma(v, u) = \alpha(v) -\alpha(u)$.% weight of the path from $v$ to $u$ equals the weight of the path from $v$ to the root minus the weight of the path from $u$ to the root.

Notice that this transformation ensures that the sibling functions of edges that belong to the same undirected edge remain anti-symmetric, because $\Delta + \gamma(v, u) = - ( -\Delta + \gamma(u,v)$. Also notice that applying the transformation rule to edges in the spanning tree naturally assigns them the identity sibling function, so they do not have to be treated separately. For intuition on the correctness, notice that the transformation preserves the length of all cycles in the jump graph.

\paragraph{Correctness of the Retemplating.}

We show that the retemplated graph instantiates an isomorphic graph, by providing a bijective function $\phi$ between the vertices of both instantiated graphs such that there is an edge in one graph if and only if there is an edge in the other graph.  We label the $i$-th instance of a vertex $v$ as $(v,i)$.

Root the spanning tree $A$ and consider $\alpha$ as above ($\alpha(v)$ is the sum of weights from $v$ to the root along $A$). For any vertex $v$ and instance number $i$, let $\phi( v, i) = \phi (v, i + \alpha(v))$. This function is bijective and its inverse is: $\phi^{-1} (v, i) = (v, i - \alpha(v)) $.

First, we map from the instantiated graph of $T$ to the instantiated graph of $T'$. Consider an edge $( (u,i), (v, j))$ in the instance of $T$. Then, this was created by an edge with a "jump" of $\Delta = j-i$. We show there is an edge $( \phi(u,i), \phi(v, j))$ in the instance of $T'$:  $( \phi(u,i), \phi(v, j)) =  ( (u,i+\alpha(u)), (v, j+\alpha(v) )$. By construction, there is an edge from $(u, i+\alpha(u))$ to $(v, i + \alpha(u) +\Delta + \gamma(v, u))$ in the instance of $T'$, which equals $(v, j + \alpha(v))$ (using $\gamma(v, u) = \alpha(v)-\alpha(u)$ and $\Delta = j-i$).

Second, we show the reverse, i.e., if there is an edge $((u, i), (v, i))$ in the instance of $T'$, then there is an edge $(\phi^{-1} (u, i), \phi^{-1} (v, j))$ in the instance of $T$. Consider an edge $((u, i), (v, j))$ in the instance of $T'$. Then, by construction of the retemplated graph, the weight $\Delta$ of the edge $(u,v)$ in the original jump graph must satisfy $i+\Delta + \alpha(v) - \alpha(u) = j$. We show there is an edge $(\phi^{-1} (u, i), \phi^{-1} (v, j))$ in the instance of $T$. $(\phi^{-1} (u, i), \phi^{-1} (v, i)) = ((u, i -\alpha(u) ), (v, j -\alpha(v))$. It remains to show $i -\alpha(u) +\Delta = j -\alpha(v)$, which follows because $\Delta = j-i-\alpha(v)+\alpha(u)$.


\subsection{Maximum Flows Revisited}

\lukas{This section contains the generalized proof for max flows}


\begin{lemma}\label{lem:stcut-structure-sibling}
In a parametric graph, if $s$ and $t$ are in the root template, there is a minimum all/once-$s$-$t$ cut that puts every instance of every vertex in the same part of the cut.
\end{lemma}

\begin{proof}
\lukas{Todo this proof should clearly distinguish when we are talking about the instantiated graph} \lukas{todo: move to ch on sibling edges}

The proof is by induction on the number of templates in the parametric graph. If the parametric graph has only a single template, then (since $s$ and $t$ must be in this template) the claim is trivial because the root is repeated only once, by assumption.

Otherwise, let $C=(V_s, V_t)$ be a minimum all-$s$-$t$ cut of the parametric graph $G$ (i.e., $V_s$ contains the vertices assigned to $s$ and $V_t$ those assigned to $t$).
%
Consider an arbitrary template $T_i$ that is a \emph{child of the root template}. Let $B_s$ and $B_t$ contain the boundary vertices of $T_i$ that are in $V_s$ and $V_t$, respectively.

If either $B_s$ or $B_t$ are empty, then it follows immediately that all instances of the vertices that are in $T_i$ are in the same part of $C$ (namely on the side of $s$ if $B_t$ is empty and vice versa).

Otherwise, merging all vertices in $B_s$ into a vertex $s'$ and merging all vertices in $B_t$ into a vertex $t'$ does not change the value of the minimum $s$-$t$ cut. Moreover, if the merged parametric graph has a minimum all-$s$-$t$ cut that puts every instance of every vertex on the same side of the cut, then so does the original parametric graph (because $B_s$ and $B_t$ contain only vertices that belong to the root template and we can "undo" the merging). We thus further assume w.l.o.g. that $B_s$ and $B_t$ contain a single vertex named $s'$ and $t'$, respectively.

Every minimum $s$-$t$ cut must separate $s'$ from $t'$ in the subgraph given by the instances of $T_i$ and the vertices $s'$ and $t'$. We use our induction hypothesis to show that there is a minimum all-$s'$-$t'$ cut in this subgraph that puts all instances of a vertex on the same side of the cut. %The cheapest way to do so is to cut every instance along a minimum $s'-t'$ cut in the subgraph induced by the instance of $T_i$ and the boundary vertices (without any edges between boundary vertices).

We construct the parametric graph $G''$ such that a maximum $s$-$t$ flow in $G''$ can be extended to a flow for all edges that intersect $G_i$ or its siblings. $G''$ has the following template graph: take the subgraph of $G$ induced by $T_i$ together with its boundary vertices, then delete any edges going $s'$ to $t'$. The boundary vertices $s'$ and $t'$ and all vertices that belong to $T_i$ are put into the root template of $G''$ (which has parameter $1$). Moreover, $G''$ has the templates and parameters of the descendants of $T_i$ in $G$. The parametric graph $G''$ contains at least one template less than $G$. Hence, by induction, there is a minimum $s'$-$t'$ cut $C''$ of $G''$ that puts all instances of the same vertex into the same partition. 

Let $f''$ bet the dual maximum $s'$-$t'$ flow corresponding to $C''$ in $G''$. Now, we construct a flow $f$ for the edges that intersect the instance $G_i$ or its siblings and show it is maximum. Along each instance of edge $e$ in $T_i$ we send $f''(e)$ flow. The capacity constraint on the flow is trivially satisfied. The conservation constraint on the flow is satisfied because the sibling functions are bijective: In the instantiated graph, the total flow going in and out of an instance of $v$ is the same as for vertex $v$ for $f''$ in $G''$. The value of the flow $f$ is $P_i \cdot v(f)$.

Now, consider the cut $C'$ were we put every instance of a vertex $v$ in $T_i$ on the same side as $v$ is in $C'$. The value of this cut is $P_i \cdot  v(f)$. By strong duality, this shows that $C$ is a minimum $s'$-$t'$ cut in the graph induced by $G_i$, its siblings, and its boundary nodes. By construction, this cut puts every instance of every vertex on the same side of the cut.

% (By contradiction: Every instance must be cut somewhere. If it is not cut along such a minimum  $P_{s}$-$P_{t}$ cut, we can make the cut cheaper by using a minimum $P_{s}$-$P_{t}$ cut.)

We conclude that all children of the root template can be cut such that every instance of the same vertex is in the same part of the cut. Because the root has a single instance, the statement follows for the root as well.

\end{proof}

\subsection{Minimum Cuts Revisited}

\lukas{This section contains the generalized (partial instantiation based) algorithm. Maybe also an FPT algorithm?}



\end{document}

